A Framework to Explore Workload-Specific Performance and Lifetime Trade-offs in Neuromorphic Computing

Neuromorphic hardware with non-volatile memory (NVM) can implement machine learning workload in an energy-efficient manner. Unfortunately, certain NVMs such as phase change memory (PCM) require high voltages for correct operation. These voltages are supplied from an on-chip charge pump. If the charge pump is activated too frequently, its internal CMOS devices do not recover from stress, accelerating their aging and leading to negative bias temperature instability (NBTI) generated defects. Forcefully discharging the stressed charge pump can lower the aging rate of its CMOS devices, but makes the neuromorphic hardware unavailable to perform computations while its charge pump is being discharged. This negatively impacts performance such as latency and accuracy of the machine learning workload being executed. In this paper, we propose a novel framework to exploit workload-specific performance and lifetime trade-offs in neuromorphic computing. Our framework first extracts the precise times at which a charge pump in the hardware is activated to support neural computations within a workload. This timing information is then used with a characterized NBTI reliability model to estimate the charge pump's aging during the workload execution. We use our framework to evaluate workload-specific performance and reliability impacts of using 1) different SNN mapping strategies and 2) different charge pump discharge strategies. We show that our framework can be used by system designers to explore performance and reliability trade-offs early in the design of neuromorphic hardware such that appropriate reliability-oriented design margins can be set.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/extra.tex <==
Aging-related defects in a charge pump are {different} from an NVM cell's endurance failures, which are due to {repeated} programming of the cell. 
\mr{
In recent prototypes, e.g. \cite{villa2018pcm}, PCM endurance is to the order of \ineq{10^{14}} cycles (\ineq{\approx} 10 years lifetime), while charge pump lifetime is only \ineq{\approx} 2-3 years at 3V.
}
Impact-wise, aging issues in a neuromorphic hardware arise during inference (reading of synaptic weights) and training (update of synaptic weights) in supervised machine learning, while endurance issues arise only during training.


%To access, i.e., read and program an NVM cell in a crossbar, its peripheral circuit drives current through the cell using a bias voltage generated from an on-chip charge pump. This voltage must be high enough to compensate for IR drop and the built-in potential of the access device, which connects the cell to a row and a column in the crossbar.

%High-voltage operations are common in neuromorphic architectures with PCM, FeRAM, and Flash NVMs, and they are generated via on-chip charge pumps built using CMOS devices \cite{Shen2018ZeroRange}. Unfortunately, when a CMOS device is stressed to a high voltage for a long duration, aging effects start to accelerate in the device, leading to negative bias temperature instability (NBTI) and hot carrier injection (HCI) generated defects \cite{gao2017nbti}. These are the dominant ones for scaled technology nodes. In older nodes, other defects such as time-dependent dielectric breakdown (TDDB) still play a role. Aging-induced defects depend on the neural activity in the SNN workload being executed on the hardware and they lower the lifetime of CMOS devices in charge pumps.

%High voltage neuromorphic operations are used in NVMs such as PCM, FeRAM, and Flash.
%, require high voltage operations for neuromorphic computing.
% is biased to a high voltage,
% %drives current (\ineq{\approx} \ineq{100\mu A} - \ineq{300\mu A}) through the cell, 
% compensating for IR drop on wires, and the built-in potential of the cell's access device, which connects the cell to a row and a column in the crossbar.
% As reported in a recent PCM prototype \cite{Kim2018EmergingComputing},
% a crossbar requires the {elevated} \ineq{1.8V} to bias its cells, \ineq{3V} to drive current through them for reading synaptic weights (stored in PCM cells) during forward propagation of neuron excitation, and \ineq{5V} to to drive current for programming them during synaptic weight updates.
%Elevated voltages in neuromorphic architectures are generated using {on-chip charge pumps}, which are
%and supplied to a crossbar via the crossbar's peripheral structures. A charge pump is 
%build using CMOS devices \cite{Shen2018ZeroRange}.

%When a CMOS device is operated at an overdrive voltage continuously for a long duration, aging effects start to appear in the device, leading to negative bias temperature instability (NBTI) generated defect and lowering the device's lifetime \cite{gao2017nbti}.
%Aging-induced defects 
%When pre-charged at these elevated voltages for {too long}, the CMOS logic {suffers} from {wear-out}, leading to time-dependent dielectric breakdown (TDDB) {failures} \cite{Gleixner2018PCMFeatures}.
%These failure mechanisms 
%are {different} from endurance failures, which are due to {repeated} programming of NVM cells.
%In neuromorphic computing, aging issues arise during inference (reading of synaptic weights) and training (update of synaptic weights) in supervised machine learning, while endurance issues arise only during training.
%In recent PCM prototypes such as \cite{Kim2018EmergingComputing}, cell endurance is estimated to the order of $10^{14}$ cycles ($\approx$ 10 years), while TDDB lifetime is only about 2-3 years at 5V. 
%So, ensuring long lifetime of charge pumps 
%by {decelerating} their aging 
%is critical because a {faulty} charge pump {cannot} provide bias voltages to crossbars, making those crossbars unusable for SNN execution.

%lower than the threshold voltage (\ineq{V_{\text{th}}})


%This performance and lifetime trade-off depends on the SNN workload that is being executed on the neuromorphic architecture.
\mrb{
This paper develops a novel framework to evaluate workload-specific performance and lifetime trade-offs in neuromorphic computing.
}
The framework incorporates the CARLsim simulator \cite{Chou2018CARLsim4} to first extract the precise time of neural activity in a network of spiking neurons in response to stimuli applied at its input for a given workload. We then propose a new analytical model that uses this spike timing to
estimate aging in charge pumps based on the synapse-to-crossbar mapping and power delivery architecture of charge pumps. We show that this framework can be integrated inside 
1) {design-time based techniques}, where neurons and synapses can be efficiently allocated to different crossbars, balancing aging of all charge-pumps, 2) {run-time based techniques}, where stressed charge pumps can be discharged at appropriate intervals, minimizing their aging without significantly impacting performance, and 3) {architectural techniques}, where a charge pump's power delivery architecture can be optimized to achieve a target lifetime. %In this paper we propose a framework to evaluate reliability and performance trade-offs specific to the workload being executed on a neuromorphic architecture.
% a design-time wear-out balancing technique and a run-time charge-pump discharge technique to explore reliability and performance trade-offs.
% We show that Our framework

% This makes them attractive for embedded and edge computing paradigms.
% A typical neuromorphic architecture consist of analog and mixed-signal neuron circuits, crossbars with non-volatile memories to store synaptic weights, and shared-interconnect to communicate spikes \cite{Burr2017NeuromorphicMemory}. We focus on those architectures whose crossbars are designed using phase-change memory (PCM) \cite{Wong2010PhaseMemory}, an emerging non-volatile memory technology. 

% PCM's cell sizes can scale down to \ineq{4F^2}, where \ineq{F} is the feature size,  allowing a very high integration density in neuromorphic architectures. This compact cell size is achieved using the Selective Epitaxial Growth (SEG) diodes \cite{Pakala2018MaterialsMemories}, which are used as access devices to PCM cells. Unfortunately, due to the diode's {high built-in potential}, the peripheral circuits in a PCM crossbar require the {elevated} 1.8V to bias these cells,  {3V} to read synaptic weights during forward propagation of neuron excitation, and {5V} to program them during (online) learning of synaptic weights for different plasticity rules.
% These elevated voltages are generated using {on-chip charge pumps}, which are cascaded resistance-capacitance circuits built using the CMOS logic \cite{Shen2018ZeroRange}.

% When precharged at the elevated voltages for {too long}, a charge pump's internal CMOS structures 
% {suffer} from {wear-out}, leading to time-dependent dielectric breakdown (TDDB) {failures} \cite{Gleixner2018PCMFeatures}.
% These are {different} from endurance failures caused by the {repeated} programming of PCM cells in a crossbar.
% In fact, 
% TDDB issues arise during both inference (reading of synaptic weights) and online learning (update of synaptic weights) in supervised machine learning approaches, whereas endurance failures arise only during online learning.
% In recent PCM prototypes such as \cite{Kim2018EmergingComputing}, cell endurance is estimated to the order of $10^{14}$ cycles ($\approx$ 10 years), while TDDB lifetime is only about 2-3 years at 5V. 
% So, ensuring long lifetime by {reducing} the TDDB-related wear-out of PCM's charge pumps is critical for neuromorphic architectures because a {faulty} charge pump {cannot} read and program PCM cells in a crossbar, which are {otherwise programmable}, making those crossbars incapable of mapping and executing neurons and synapses.

% \begin{figure*}[t!]
% 	\centering
% 	%\vspace{-10pt}
% 	\centerline{\includegraphics[width=1.99\columnwidth]{images/overview_pcm.pdf}}
% 	\caption{Overview of how a PCM cell is used in a neuromorphic architecture to execute SNNs.}
% 	\vspace{-10pt}
% 	\label{fig:overview_pcm}
% \end{figure*}


% NBTI aging issues in neuromorphic architectures can be mitigated using 1) \textbf{design-time based techniques}, where neurons and synapses can be efficiently allocated to different crossbars, balancing aging of all charge-pumps, 2) \textbf{run-time based techniques}, where stressed charge pumps can be discharged at appropriate intervals, minimizing their aging without significantly impacting performance, and 3) \textbf{architectural techniques}, where a charge pump's power delivery load can be optimized to achieve a target operating lifetime. In this paper we propose a framework to evaluate reliability and performance trade-offs specific to the workload being executed on a neuromorphic architecture.

% In this paper we propose a novel framework to estimate wear-out of on-chip charge-pumps during neuromorphic computing. This framework incorporates the CARLsim simulator \cite{Chou2018CARLsim4} to first extract the precise time of neural activity in a network of spiking neurons in response to changing stimuli applied at its input. We then propose a new TDDB-related wear-out model that uses this spike timing to
% estimate wear-out in charge pumps based on the synapse-to-crossbar mapping and the power delivery load of charge pumps. We show that this framework can be used in a design-time wear-out balancing technique and a run-time charge-pump discharge technique to explore reliability and performance trade-offs.
%information together with 1) material parameters of PCM and 2) the placement information comprising of synapse-to-crossbar mapping to estimate wear-out of charge pumps in neuromorphic architectures when executing SNNs.
%our new reliability model estimates TDDB-related wear-out in charge pumps.
%in the architectures due to neural activities in SNN-based applications.
%We demonstrate how this novel framework can be integrated in design-time based techniques, run-time based techniques and architectural techniques for lifetime optimizations.
%Using this wear-out estimate and its relationship to the operating lifetime, measured as the mean-time-to-failure (MTTF), we can apply several optimization strategies such as adapting the synapse placement, controlling the discharge of charge-pumps, and optimizing the charge-pump related architectural decisions to maximize or achieve a target lifetime.

% This paper is organized as follows. We provide a brief background of spiking neural networks and how they are mapped to neuromorphic architectures in Section \ref{sec:background}. We introduce our reliability assessment framework in Section \ref{sec:reliability} introducing our new reliability model. We then use this framework to evaluate 1) design-time synapse placement decisions in Section \ref{sec:design_time}, 2) run-time performance-reliability trade-offs in discharging precharged charge pumps in Section\ref{sec:run_time}, and 3) lifetime due to different architectural design decisions in Section \ref{sec:architecture}. We conclude the paper and provide an outlook of our future work in Section \ref{sec:conclusion}.

==> sections/junk.tex <==
\mr{hardware such as TrueNorth \cite{DeBole2019TrueNorth:Years}, Loihi \cite{Davies2018Loihi:Learning}, and DynapSE \cite{Moradi2018ADYNAPs} can execute spiking neural networks (SNNs) \cite{Maass1997NetworksModels} in an energy efficient manner.
}
A typical neuromorphic hardware consists of \textit{artificial neurons}, which generate spikes when a neuron's action potential exceeds a threshold and \textit{crossbars} with non-volatile memory (NVM) cells, which store synaptic weights \cite{Burr2017NeuromorphicMemory}. 
%Each crossbar has a peripheral circuit to drive current for reading and programming synaptic weights.% based on spikes generated from neurons in the architecture.
%in crossbars, and 4) a shared interconnect for communicating spikes between crossbars \cite{Burr2017NeuromorphicMemory}.
\mr{
To implement neural computations, an NVM cell such as phase-change memory (PCM), ferroelectric RAM (FeRAM), and Flash requires high voltages, which are supplied from on-chip charge pumps of the hardware \cite{Shen2018ZeroRange}.
When operating at these voltages, a charge pump's internal CMOS devices are stressed. One example is the threshold voltage (\ineq{V_\text{th}}) shift. 
If the charge pump is activated too frequently, its CMOS devices do not recover from stress, accelerating their \textit{aging} and eventually leading to charge pump failures.
}

% let \ineq{\mathcal{A}_{s}} be the aging of the charge pump to process spike train \ineq{\{\tau_1^s,\tau_2^s,\cdots,\tau_{k_s}^s\}} on the \ineq{s^\text{th}} synapse, \ineq{C} be the number of crossbars and \ineq{L} the number of charge pumps in the neuromorphic architecture. Let \ineq{\mathcal{M} \in \mathbb{R}^{S\times C}} be the synapse-to-crossbar mapping and \ineq{\mathcal{P}\in \mathbb{R}^{C\times L}} be the crossbar-to-charge pump power delivery architecture, defined as

% Lifetime of a charge pump is measured in terms of its \emph{Mean Time To Failure} (MTTF), which for TDDB-related failure mechanism can be expressed as follows \cite{kauerauf2011methodologies}.
% \begin{equation}
% \label{eq:mttf_tddb}
% \scriptsize MTTF = A.e^{-\gamma\sqrt{V}},
% \end{equation}
% where \ineq{V} is the operating voltage, and \ineq{A} and \ineq{\gamma} are the material-related constants. 
% TDDB failures can also be modeled using the Weibull distribution \cite{fenner2018making} with a scale parameter \ineq{\alpha} and a slope parameter \ineq{\beta}. The reliability at time \ineq{t} is
% \begin{equation}
% \label{eq:eq1}
% \scriptsize R(t) = e^{-\left(\frac{t}{\alpha(V)}\right)^\beta}, \text{ and } MTTF = \int_{0}^{\infty}R(t)dt = \alpha(V)\Gamma\left(1+ \frac{1}{\beta}\right),
% \end{equation}
% where \ineq{\Gamma} is the Gamma function. Equating Equations \ref{eq:mttf_tddb} \& \ref{eq:eq1},
% % and rearranging, we can express the scale parameter \ineq{\alpha} as
% %Using Eq. \ref{eq:mttf_tddb}, and rearranging.
% \begin{equation}
% \label{eq:eq3}
% \scriptsize \alpha(V) = \frac{A.e^{-\gamma\sqrt{V}}}{\Gamma\left(1+\frac{1}{\beta}\right)}.
% \end{equation}
% We divide the SNN execution time \ineq{[0,T]} into \ineq{m} equal intervals \ineq{0 = t_0 < t_1 \cdots<t_m = T}, with \ineq{[t_i,t_{i+1})} as the \ineq{(i+1)^{\text{th}}} interval and \ineq{V_i} is the charge pump's voltage in this interval.

% We use \cite{das2015reliability} to formulate reliability (derivations omitted for space limitations) at the end of SNN execution as
% \begin{equation}
% \label{eq:eq10}
% \scriptsize R(T) = e^{-\left(\sum_{i=0}^{m-1}\frac{\Delta t_i}{\alpha(V_i)}\right)^{\beta}}.
% \end{equation}

% The reliability at the start and end of the first interval is
% \begin{equation}
% \label{eq:eq4}
% \scriptsize R(t)|_{t=t_0} = 1, \text{~~~~and~~~~} R(t_1^-) = e^{-\left(\frac{t_1}{\alpha(V_0)}\right)^\beta}.
% \end{equation}
% Using the term \ineq{\theta} to represent the wear-out of the charge pump in the interval \ineq{[t_o,t_1)}, the reliability of the charge pump at the beginning of the second interval is
% \begin{equation}
% \label{eq:eq7}
% \scriptsize R(t_1^+) = e^{-\left(\frac{t_1+\theta}{\alpha(V_1)}\right)^\beta}.
% \end{equation}
% To maintain continuity of reliability at the end of first interval and the beginning of second interval, we equate Equations \ref{eq:eq4} \& \ref{eq:eq7} to compute \ineq{\theta} as
% \begin{equation}
% \label{eq:eq8}
% \scriptsize \theta = \left(\frac{\alpha(V_1)}{\alpha(V_0)} - 1\right)t_1.
% \end{equation}
% Substituting this expression of \ineq{\theta} in Equation \ref{eq:eq7}, reliability at time \ineq{t_2} can be expressed as 
% \begin{equation}
% \label{eq:eq9}
% \scriptsize R(t_2) = e^{-\left(\frac{\Delta t_1}{\alpha(V_1)} + \frac{\Delta t_0}{\alpha(V_0)}\right)^{\beta}}.
% \end{equation}
% We can extend this equation to compute reliability at the end of the SNN execution as
% \begin{equation}
% \label{eq:eq10}
% \scriptsize R(T) = e^{-\left(\sum_{i=0}^{m-1}\frac{\Delta t_i}{\alpha(V_i)}\right)^{\beta}}.
% \end{equation}

%where \ineq{\alpha(V_i)} is calculated using Equation \ref{eq:eq3}.

%Equation \ref{eq:eq11} computes the wear-out of a charge pump for its voltage profile (e.g., Figure \ref{fig:cp_motivate}(b)) needed to process a spike train (e.g., Figure \ref{fig:cp_motivate}(a)). 

% \begin{equation}
% \label{eq:eq10}
% \scriptsize R(T) = e^{-\left(\sum_{i=0}^{m-1}G(V_i)\right)^{\beta}},
% \end{equation}

%\ineq{\beta} is the shape parameter of the NBTI defect distribution and 

==> sections/reliability.org..tex <==
We introduce our framework for \textit{PCM crossbars considering NBTI aging}. The framework can be extended for other NVMs such as FeRAM and Flash, where high voltage operations lead to aging issues. The framework can also model aging due to other generated defects such as TDDB and HCI.

% A charge pump's lifetime is typically a few years, which is much longer than the execution time of an SNN.
% To estimate how much a charge pump's lifetime degrades during an SNN's execution time, 
% we estimate the charge pump's wear-out in this duration and use it to extrapolate lifetime, assuming the SNN is executed repeatedly until the charge pump fails due to TDDB failure. Therefore, improving a charge pump's lifetime is the same as reducing its wear-out during the . 
\textbf{Aging Model --} Lifetime of a charge pump is measured in terms of its \emph{Mean Time To Failure} (MTTF), which for TDDB-related failure mechanism can be expressed as follows \cite{kauerauf2011methodologies}.
\begin{equation}
\label{eq:mttf_tddb}
\scriptsize MTTF = A.e^{-\gamma\sqrt{V}},
\end{equation}
where \ineq{V} is the operating voltage, and \ineq{A} and \ineq{\gamma} are the material-related constants. 
TDDB failures can also be modeled using the Weibull distribution \cite{fenner2018making} with a scale parameter \ineq{\alpha} and a slope parameter \ineq{\beta}. The reliability at time \ineq{t} is
\begin{equation}
\label{eq:eq1}
\scriptsize R(t) = e^{-\left(\frac{t}{\alpha(V)}\right)^\beta}, \text{ and } MTTF = \int_{0}^{\infty}R(t)dt = \alpha(V)\Gamma\left(1+ \frac{1}{\beta}\right),
\end{equation}
where \ineq{\Gamma} is the Gamma function. Equating Equations \ref{eq:mttf_tddb} \& \ref{eq:eq1},
% and rearranging, we can express the scale parameter \ineq{\alpha} as
%Using Eq. \ref{eq:mttf_tddb}, and rearranging.
\begin{equation}
\label{eq:eq3}
\scriptsize \alpha(V) = \frac{A.e^{-\gamma\sqrt{V}}}{\Gamma\left(1+\frac{1}{\beta}\right)}.
\end{equation}
We divide the SNN execution time \ineq{[0,T]} into \ineq{m} equal intervals \ineq{0 = t_0 < t_1 \cdots<t_m = T}, with \ineq{[t_i,t_{i+1})} as the \ineq{(i+1)^{\text{th}}} interval and \ineq{V_i} is the charge pump's voltage in this interval.

We use \cite{das2015reliability} to formulate reliability (derivations omitted for space limitations) at the end of SNN execution as
\begin{equation}
\label{eq:eq10}
\scriptsize R(T) = e^{-\left(\sum_{i=0}^{m-1}\frac{\Delta t_i}{\alpha(V_i)}\right)^{\beta}}.
\end{equation}

% The reliability at the start and end of the first interval is
% \begin{equation}
% \label{eq:eq4}
% \scriptsize R(t)|_{t=t_0} = 1, \text{~~~~and~~~~} R(t_1^-) = e^{-\left(\frac{t_1}{\alpha(V_0)}\right)^\beta}.
% \end{equation}
% Using the term \ineq{\theta} to represent the wear-out of the charge pump in the interval \ineq{[t_o,t_1)}, the reliability of the charge pump at the beginning of the second interval is
% \begin{equation}
% \label{eq:eq7}
% \scriptsize R(t_1^+) = e^{-\left(\frac{t_1+\theta}{\alpha(V_1)}\right)^\beta}.
% \end{equation}
% To maintain continuity of reliability at the end of first interval and the beginning of second interval, we equate Equations \ref{eq:eq4} \& \ref{eq:eq7} to compute \ineq{\theta} as
% \begin{equation}
% \label{eq:eq8}
% \scriptsize \theta = \left(\frac{\alpha(V_1)}{\alpha(V_0)} - 1\right)t_1.
% \end{equation}
% Substituting this expression of \ineq{\theta} in Equation \ref{eq:eq7}, reliability at time \ineq{t_2} can be expressed as 
% \begin{equation}
% \label{eq:eq9}
% \scriptsize R(t_2) = e^{-\left(\frac{\Delta t_1}{\alpha(V_1)} + \frac{\Delta t_0}{\alpha(V_0)}\right)^{\beta}}.
% \end{equation}
% We can extend this equation to compute reliability at the end of the SNN execution as
% \begin{equation}
% \label{eq:eq10}
% \scriptsize R(T) = e^{-\left(\sum_{i=0}^{m-1}\frac{\Delta t_i}{\alpha(V_i)}\right)^{\beta}}.
% \end{equation}
We introduce the term \emph{aging} \ineq{\mathcal{A}} as a measure of wear-out in the pre-charged charge pump due to TDDB failures as
\begin{equation}
\label{eq:eq11}
\scriptsize \mathcal{A} = \sum_{i=0}^{m-1}\frac{\Delta t_i}{\alpha(V_i)}, \text{ such that } R(T) = e^{-\mathcal{A}^{\beta}}.
\end{equation}
%where \ineq{\alpha(V_i)} is calculated using Equation \ref{eq:eq3}.

%Equation \ref{eq:eq11} computes the wear-out of a charge pump for its voltage profile (e.g., Figure \ref{fig:cp_motivate}(b)) needed to process a spike train (e.g., Figure \ref{fig:cp_motivate}(a)). 

Equation \ref{eq:eq11} is derived considering all synapses of the SNN are mapped to the same crossbar, which is powered by a single charge pump. In practical scenarios, 1) synapses are distributed across different crossbars of the architecture because a crossbar can accommodate only a limited number of synapses and 2) a neuromorphic architecture integrates more than one charge pump to balance the power delivery to different crossbars. We now describe how to extend Equation \ref{eq:eq11} to incorporate the practical constraints of neuromorphic architectures. 

We consider the SNN \ineq{\mathcal{G}}, with \ineq{N} neurons and \ineq{S} synapses, excited with an input over the time interval \ineq{[0,T]}. 
%Neural activities in this time interval generate spikes. 
We arrange the spikes in this interval by synapses they excite as
\begin{equation}
    \label{eq:spike_time_synapse}
    \footnotesize \mathcal{S} = \{\tau_1^1,\tau_2^1,\cdots,\tau_{k_1}^1\},\{\tau_1^2,\tau_2^2,\cdots,\tau_{k_2}^2\},\cdots,\{\tau_1^S,\tau_2^S,\cdots,\tau_{k_S}^S\}, %\text{ where }
\end{equation}
where \ineq{\tau_j^s} is the \ineq{j^\text{th}} spike on \ineq{s^\text{th}} synapse of the SNN. Let \ineq{\mathcal{A}_{s}} be the charge pump's wear-out to process spike train \ineq{\{\tau_1^s,\tau_2^s,\cdots,\tau_{k_s}^s\}} on the \ineq{s^\text{th}} synapse. Let \ineq{C} be the number of crossbars and \ineq{L} the number of charge pumps in the neuromorphic architecture. Let \ineq{\mathcal{M} \in \mathbb{R}^{S\times C}} be the synapse-to-crossbar mapping and \ineq{\mathcal{P}\in \mathbb{R}^{C\times L}} be the crossbar-to-charge pump power delivery architecture, defined as
\begin{equation}
    \label{eq:mapping}
    \footnotesize m_{ij}\in \mathcal{M} = \begin{cases}
    1 & \text{if synapse } i \text{ is mapped to crossbar } j\\
    0 & \text{otherwise}
    \end{cases}
\end{equation}

\begin{equation}
    \label{eq:placement}
    \footnotesize p_{jk}\in \mathcal{P} = \begin{cases}
    1 & \text{if crossbar } j \text{ is powered by charge pump } k\\
    0 & \text{otherwise}
    \end{cases}
\end{equation}

Combining these two equations, we generate the synapse-to-charge pump mapping as
\begin{equation}
    \label{eq:placement}
    \footnotesize m_{ij}\cdot p_{jk} = \begin{cases}
    1 & \text{if synapse } i \text{ is powered by charge pump } k\\
    0 & \text{otherwise}
    \end{cases}
\end{equation}

The total wear-out of charge pump \ineq{k} is therefore
\begin{equation}
    \label{eq:wear_out_cp}
    \footnotesize \text{wear-out}_k = \sum_{i=1}^S \sum_{j=1}^C m_{ij}\cdot p_{jk}\cdot \mathcal{A}_i
\end{equation}

\begin{figure}[t!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/framework.pdf}}
	\caption{Proposed framework.}
	\vspace{-20pt}
	\label{fig:framework}
\end{figure}

\noindent \textbf{Proposed Framework --} Figure \ref{fig:framework} illustrates our framework to evaluate wear-out of charge pumps in a neuromorphic architecture.
We use the CARLsim simulator \cite{Chou2018CARLsim4} to train a SNN using the training and validation data
%, which are representative of the data that the SNN will encounter during inference. 
Apart from the trained model, CARLsim also generates \ineq{\mathcal{S}}, the precise time of spike on all synapses of the SNN. A SNN mapping approach such as \cite{das2018mapping} uses CARLsim output to generate the synapse-to-crossbar mapping \ineq{\mathcal{M}}, optimizing some objective function. In \cite{das2018mapping}, the objective function is to minimize the number of spikes communicated between crossbars, which leads to lower energy and latency on the shared interconnect. Once the SNN is mapped to crossbars of the architecture, performance of the SNN is obtained in terms of inter-spike interval \ineq{\mathcal{I}} (see Equation \ref{eq:isi}).

Using this synapse-to-crossbar mapping and the crossbar-to-charge pump connectivity, which is specific to the neuromorphic architecture, our novel formulation (Equation \ref{eq:wear_out_cp}) evaluates the wear-out of all charge pumps in the architecture when executing the SNN. This design flow is indicated using solid arrows in Figure \ref{fig:framework}.

Figure \ref{fig:framework} also illustrates three future directions based on this framework using the dashed arrows.
First, wear-out can be used in the SNN mapping step to balance wear-out of different charge pumps in the architecture. This is shown by the dashed arrow labeled \emph{wear-out-aware mapping}. Second, the crossbar-to-charge pump connectivity can be optimized to achieve a desired lifetime of charge pumps for executing an SNN. This is shown using the dashed line labeled \emph{application-specific charge pump placement}. Third, strategies can be developed to discharge charge pumps at run-time to improve their lifetime. This is shown in the \emph{Discharge Management} step. 

%In this paper, we implement these techniques and illustrate how they impact wear-out and performance. 
